Developing and Deploying a Taxi Price Comparison Mobile App in the Wild: Insights and Challenges

As modern transportation systems become more complex, there is need for mobile applications that allow travelers to navigate efficiently in cities. In taxi transport the recent proliferation of Uber has introduced new norms including a flexible pricing scheme where journey costs can change rapidly depending on passenger demand and driver supply. To make informed choices on the most appropriate provider for their journeys, travelers need access to knowledge about provider pricing in real time. To this end, we developed OpenStreetcab a mobile application that offers advice on taxi transport comparing provider prices. We describe its development and deployment in two cities, London and New York, and analyse thousands of user journey queries to compare the price patterns of Uber against major local taxi providers. We have observed large heterogeneity across the taxi transport markets in the two cities. This motivated us to perform a price validation and measurement experiment on the ground comparing Uber and Black Cabs in London. The experimental results reveal interesting insights: not only they confirm feedback on pricing and service quality received by professional drivers users, but also they reveal the tradeoffs between prices and journey times between taxi providers. With respect to journey times in particular, we show how experienced taxi drivers, in the majority of the cases, are able to navigate faster to a destination compared to drivers who rely on modern navigation systems. We provide evidence that this advantage becomes stronger in the centre of a city where urban density is high.

==> feedback.tex <==
% \subsection{Community Feedback}
Apart from quantitatively analyzing the data collected, a core goal of our service has been the interaction with the users and the taxi driver community. Both groups reached out through the application's feedback system to share their views, provide suggestions for new features or criticize the accuracy of the app's estimates. %This feedback has been very valuable in improving the app service.
Next we summarize the feedback received at the various stages as well as how this helped in the construction of our experiment which we describe in Section~\nameref{sec:experiment}.
Users also submitted reviews in the two app stores that provided essential information on bugs which were not caught during the testing phase of the app we run locally. 

%During this process we have learned about issues both regarding the app and taxi transport more generally that it would be hard to know through other means. This interaction has helped us improve the app's in various fronts as we describe below.
%Next we provide what we have considered to be a key subset of the hundreds of comments received by users and drivers in both cities and narrate how they have speficially
%led us to take new development decisions and moreover have motivate us to run an experiment that follows in 
%Section~\ref{sec:experiment}.
\paragraph*{User Feedback}


\textbf{Geographic Expansion}:
After our first deployment in New York, one of the most common requests we have received has been for expansion of our application in cities outside New York. 

\begin{framed}
Please expand outside New York (Justin, U.S.A.)
\end{framed}

In our very first deployment we used an open dataset 
shared in New York city by the local taxi authorities~\cite{TLCTrips}.
The data describes journeys and corresponding prices for millions of trips in the city between 2009 and 2015. Our estimates were provided by aggregating historic taxi journeys in 100 meter vicinity to the origin and destination points and 
returning their mean price value.
A critical obstacle to expand in other cities has been the lack of open and freely available datasets on taxi mobility and pricing. Hence, integrating the HERE Maps API (as described in Section~\ref{sec:analysis}) in route estimation allowed us to launch in London and we plan to reach new cities in the following versions of the app.

% we had to make use of an external API (Taxi Fare Finder) which is available for other cities too~\cite{taxifarefinder}. Whereas the API provides large geographic coverage as we discuss next it also suffers from inaccurate estimates that have been picked up by our user community and have helped us improve journey estimates.

\textbf{Presenting Prices}:
In the first version of the application (New York deployment only) we did not provide price estimates to users.
% were also reluctant to provide estimates on prices as we considered the risk of providing 
% financial consultantion to users too high, given the uncertainty of predicting vehicle travel times, routes and prices. \cm{I would not talk about risks as then we decided to do, I would cut this and simply said we did not provide estimates}
Instead we provided only a recommendation on the cheapest provider. However, users requested specific price estimates as the two representative
comments suggest below.
\begin{framed}
Instead if just the winner, can you also show the price details? (Anonymous User, New York)
\end{framed}
\begin{framed}
Love the app..!! Would be useful to have an estimate of the price difference between taxi and uber when the recommendation is given. (Anonymous User, New York)
\end{framed}
Hence a few months after our first launch we integrated the price estimation feature too. We highlighted nonetheless that the prices shown were estimates and encouraged
our users to come back to us with feedback on estimates that deviated from actual fares. 

\textbf{Extra Costs}:
Users responded sometimes providing surprising insights on extra costs that where added to their standard fare.
One example is shown below where airport transport resulted to an additional fee and toll charge for a user in New York.   
\begin{framed}
From 569 Lexington Ave to Laguardia Airport. Your estimate: $38$ Actual: $52$
It looked like $38$ was about correct for mileage and time but going to the airport they added a fee, plus tolls.
(Haley, User, New York).
\end{framed}
The above reveals how challenging the design of a generalizable API for taxi journeys can be. Specific charges and when they
are applied can depend on regulations applied by local transport authorities and even within the same city
extra charges can change over time, for instance during Christmas or Easter holidays. As it has been the case for many real world 
systems described online such as mapping tools and location-based services, crowdsourcing and integration of user feedback more in general could be a promising method to build large scale transport APIs that provide accurate information. Our system is one step in this direction.

\paragraph*{Driver Feedback}
Another valuable source of feedback has been the community of Black Cab drivers in London, a city where at launch we received a considerably large number of comments on overestimating the journeys of Black Cabs. Expert driver feedback has been extremely valuable and provided rare insights on journey and routing behaviors. As some of the feedback has highlighted some deep inaccuracies, this pushed us to run price validation tests (which will be described in Section~\nameref{sec:experiment}).
%However, input here has be taken into account with care as their views are more likely to be biased since opinions may reflect personal interest. 
As discussed below, some of the drivers have volunteered
to do tests on the app's accuracy for multiple routes. Other views were somewhat emotionally charged, which has been understandable. We note that we received no feedback from drivers in New York. Perhaps this is due the fact that drivers in London typically own their cabs, whereas in New York in most cases they are employed by a larger corporation. A few representative cases of driver input are discussed below. 

\textbf{Favouring Uber}:
A Black Cab driver suggested that our app is in support of Uber.    
\begin{framed}
I find your estimated prices very inaccurate with regards to black cab. Journey from Kings St to W12 9ba costs \pounds 8 in black cab instead of \pounds 19 that you estimated. This app favors uber.(Goran, Driver, London).  
\end{framed}
While this feedback could indeed reflect a very bad estimate provided through the app, we could not be sure of its honesty. Section~\nameref{sec:experiment} describes how we decided to address this comment with a validation experiment.
% as it comes from a driver that is associated with a specific provider and has a particularly aggressive tone.

\textbf{Volunteer Tester}:
In another occasion, we received metered validation tests run by a driver for a number of routes.
\begin{framed}
Your taxi fares estimate always seems high. There are a few regular journeys I inputted and did the same with quite a few jobs and every time I have come in under your taxi estimate.

3 examples were:
New Kings Rd, SW6 to Grovesnor Crescent, SW1, usually \pounds 9, your app says 11 \pounds,
Belgrave Sq, SW1 to Heathrow Terminal 5 usually \pounds 55, your app says 60 \pounds,
New Kings Rd to Canary Wharf usually \pounds 38 when your app says 40 \pounds. (Ross, Driver, London).
\end{framed}
Following his suggestion in addition to others 
we decided to reduce estimates for Black Cabs by adding a multiplier coefficient of $0.9$ (reduction by $10$\%). As we validate in Section~\ref{sec:experiment}, the correction has improved predictions overall. 

We then asked the same driver to run a few more tests and provide feedback.
\begin{framed}
I compared your estimates with about 10 jobs I done today and your pretty much spot on. A couple were pounds 1-2 over, a couple were under and some were on the button!

Another thing I thought of is to maybe let people know that these estimates are for the Taxi day rate (rate 1) and for Uber without a surge price in effect.

For taxis there are 3 rates, rate 1 from 06:00-20:00, rate 2 from 20:00-22:00 and rate 3 from 22:00-06:00. To be honest there isn't much difference between rates 1 and 2, but rate 3 does make it a bit more expensive.

(Ross, Driver, London).
\end{framed}
While map APIs provide information on shortest routes given origin and destination information, also taking into account real time traffic information as HERE Maps or Google Maps do, these systems are configured to reflect the behavior of a regular car drivers. 

We hypothesize that this may not necessarily reflect the routing and driving capabilities of professional drivers.
Furthermore, many Black Cab drivers mentioned that they do not use a navigation system as they know whereabouts in the city well through training and experience. To shed more light on these matters we run a measurement and validation experiment on taxi providers in London that we present in the following section.

% \begin{itemize}
% \item add rafar comment on sat nav
% \end{itemize}



